An Embedded Monocular Vision Approach for Ground-Aware Objects Detection and Position Estimation

In the RoboCup Small Size League (SSL), teams are encouraged to propose solutions for executing basic soccer tasks inside the SSL field using only embedded sensing information. Thus, this work proposes an embedded monocular vision approach for detecting objects and estimating relative positions inside the soccer field. Prior knowledge from the environment is exploited by assuming objects lay on the ground, and the onboard camera has its position fixed on the robot. We implemented the proposed method on an NVIDIA Jetson Nano and employed SSD MobileNet v2 for 2D Object Detection with TensorRT optimization, detecting balls, robots, and goals with distances up to 3.5 meters. Ball localization evaluation shows that the proposed solution overcomes the currently used SSL vision system for positions closer than 1 meter to the onboard camera with a Root Mean Square Error of 14.37 millimeters. In addition, the proposed method achieves real-time performance with an average processing speed of 30 frames per second.

==> content/acknowledgement.tex <==
\section{Acknowledgement}

%We would like to first thanks to our advisors and the Informatic Center - UFPE (Centro de Informática (CIn) - UFPE) for all the support and knowledge during this year of project and development. We also would like to thanks all the help from our sponsors: In Loco, Neurotech, Maxon Group, HSBS, In Forma, Maedler, Altium, CI Intercâmbio e Viagem, Lierre and Instituto Nacional de Tecnologia em União e Revestimento de Materiais (INTM).

==> content/others.tex <==

\begin{comment}
\section{Omnidirectional Mobile Robot Model} \label{ch2}


To develop a no-slip control system, first, we have to derive a mathematical model of the robot. The kinematics model tells how to control the robot's movement's speed and direction in a global frame. With the kinematic model, it is possible to set each wheel's speed to make the robot move in a particular direction. On the other hand, the dynamics model tells how the forces impact the robot's movement. With the dynamic model, it is possible to prevent wheel slippage and identify how it acts on the robot. Figure \ref{fig:kin3} shows an omnidirectional mobile robot with four wheels which moves in a global reference frame local reference frame $\{X_I,Y_U\}$ through movements in its local reference frame $\{X_R,Y_R\}$ with a displacement angle $\theta$.


\begin{figure}
\centering
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=.82\linewidth]{imgs/3_kinematics3.png}
  \caption{Global and local reference frames.}
  \label{fig:kin3}
\end{minipage}%
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=0.95\linewidth]{imgs/2_kinematics2.png}
  \caption{Parameters of an omnidirectional wheel.}
  \label{fig:kin1}
\end{minipage}
\end{figure}



\subsection{Kinematic Model}

To build an omnidirectional mobile robot kinematic model, we have to derive the constraints for each wheel. Figure \ref{fig:kin1} depicts an omnidirectional wheel with its kinematic parameters. According to Siegwart \cite{Siegwart:2011}, the motion constraints for an omnidirectional wheel are described in equation (\ref{eq:kin1}):

\begin{equation}\label{eq:kin1}
\begin{bmatrix}
    sin(\alpha+\beta+\gamma) & -cos(\alpha+\beta+\gamma) & (-l)cos(\beta+\gamma)
\end{bmatrix}
     R(\theta)\dot{\xi_I} - r\dot{\phi}cos(\gamma) = 0
\end{equation}

The first term is a three-element vector that maps the contribution for motion on the wheel plane. The rotation matrix, $R(\theta)$, transforms the motion parameters, $\dot{\xi_I}$, from the global reference frame $\{X_I,Y_I\}$ to the local reference frame $\{X_R,Y_R\}$. The wheel parameters $\alpha$, $\beta$, $\gamma$ are the angle between the wheel and the local reference frame axis, wheel to chassis relative angle, and wheel to roller rotation axis angle, respectively. The wheel has a radius $r$ and angular speed $\dot{\phi}$.

For this application, we consider an omnidirectional mobile robot under the RoboCup SSL competition rules, as shown in Figure \ref{fig:kin2}. The robot has four omnidirectional wheels, and the value of the movement speed in the global reference frame can be calculated using equation (\ref{eq:kin2}):

\begin{figure}[ht]
\centering
\includegraphics[width=.50\textwidth]{imgs/1_kinematics1.png}
\caption{Omnidirectional Mobile Robot Kinematic Parameters in a Small Size League Robot.}
\label{fig:kin2}
\end{figure} 

\begin{equation}\label{eq:kin2}
     \dot{\xi_I} = R(\theta)^{-1}{J_{1f}^{-1}}J_2\dot{\phi}
\end{equation}

The matrix $J_{1f}$ is an extension of the first matrix of equation (\ref{eq:kin1}) for the four omnidirectional wheels with $90^{\circ}$. $J_2$ is a diagonal matrix with the wheel radius, and $\dot{\phi}$ is now a matrix with each wheel's angular speeds. Therefore, it is possible to relate each wheel's desired speed to the robot's overall speed. Rearranging the equation (\ref{eq:kin2}) to find the speed of each wheel, we have the equation (\ref{eq:kin3}):

\begin{equation}\label{eq:kin3}
     \Dot{\phi}= 
     \begin{bmatrix}
        \Dot{\phi_1} \\
        \Dot{\phi_2} \\
        \Dot{\phi_3} \\
        \Dot{\phi_4}
     \end{bmatrix}
     = J_2^{-1}J_{1f}R(\theta)\Dot{\xi_I} 
\end{equation}

Expanding each matrix's terms, we have the kinematics model for an omnidirectional mobile robot with four wheels. The reference value for each wheel for the robot to move with speeds $\Dot{x}$, $\Dot{y}$ and $\Dot{\theta}$ in the global reference frame is given by equation (\ref{eq:kin4}):

\begin{equation} \label{eq:kin4}
    \Dot{\phi}=    
    \begin{bmatrix}
        \frac{1}{r} && 0 && 0 && 0 \\
        0 &&  \frac{1}{r} && 0 && 0 \\
        0 && 0 &&  \frac{1}{r} && 0\\
        0 && 0 && 0 &&  \frac{1}{r}
    \end{bmatrix}
    \begin{bmatrix}
        -sin(\alpha_1)  && cos(\alpha_1) && l \\
        -sin(\alpha_2)  && cos(\alpha_2) && l \\
        sin(\alpha_3)   && cos(\alpha_3) && l \\
        sin(\alpha_4)   && cos(\alpha_4) && l
    \end{bmatrix}
    \begin{bmatrix}
        cos\theta & sin\theta & 0 \\
      -sin\theta & cos\theta & 0 \\
        0 & 0 & 1
    \end{bmatrix} 
    \begin{bmatrix}
        \Dot{x} \\
        \Dot{y} \\
        \Dot{\theta}
    \end{bmatrix}
\end{equation}

The specific parameters for the omnidirectional mobile robot designed under the SSL rules used in this paper are in Table (\ref{table:kin1}).

\begin{table}[!htb]
\centering
\caption{Robot Kinematic and Dynamic Parameters} 
\begin{tabular}{ccc} \label{table:kin1} \\
\hline
\textbf{Parameter}  & \textbf{Description}      & \textbf{Value}     \\  \hline
$\alpha_1$          & Wheel angle for motor 1 (in degrees)  &   $60$        \\
$\alpha_2$          & Wheel angle for motor 2 (in degrees)  &   $135$       \\
$\alpha_3$          & Wheel angle for motor 3 (in degrees)  &   $135$       \\
$\alpha_4$          & Wheel angle for motor 4 (in degrees)  &   $60$        \\
$\beta$             & Wheel plane to robot chassis angle (in degrees)    &   $0$         \\
$\gamma$            & Wheel plane to roller axis angle (in degrees)   &   $0$     \\
$r$                 & Wheel radius (in meters)             & $0.02425$         \\
$l$                 & Distance from robot center to wheel (in meters) & $0.081$           \\
$M$                 & Robot's total weight (in kilograms)     & 2.53  \\
$\Delta x$          & Center of mass  x distance from geometric center (in meters) & $-0.0014$ \\
$I$                 & Robot's moment of inertia (in $kg\cdot m^2$) & 0.0173\\
$\dot{x}_{max}$     & Robot's maximum speed in x axis (in m/s)    & 3 \\
$\dot{x}_{max}$      & Robot's maximum speed in y axis (in m/s) & 3 \\
$\dot{\theta}_{max}$    & Robot's maximum angular speed (in rad/s)  & 30 \\
\hline
\end{tabular}
\end{table}


\subsection{Dynamic Model}

For building an omnidirectional mobile robot dynamic model, the forces acting in each wheel need to be determined. When considering a robot in movement with the arrangement in Figure \ref{fig:kin2}, there is a force with magnitude $F_i$ in each $i$ wheel, which will move the robot center of mass with a specific translational acceleration $\Ddot{x}$, $\Ddot{y}$ and an angular acceleration $\Ddot{\theta}$. The relation between this acceleration and the robot's forces is given by a matrix called force coupling matrix \cite{Rojas:2006}. The dynamic model for an omnidirectional mobile robot with four wheels is given by equation (\ref{eq:dyn1}):

\begin{equation} \label{eq:dyn1}
        \begin{bmatrix}
        \Ddot{x} \\
        \Ddot{y} \\
        \Ddot{\theta}
    \end{bmatrix}=   \frac{1}{M}
    \begin{bmatrix}
        -sin(\alpha_1)  && -sin(\alpha_2) && sin(\alpha_3) && sin(\alpha_4)  \\
        cos(\alpha_1)  && cos(\alpha_2) &&  cos(\alpha_3) && cos(\alpha_4) \\
        \frac{Ml}{I}   && \frac{Ml}{I}  &&  \frac{Ml}{I}  &&  \frac{Ml}{I} 
    \end{bmatrix}
    \begin{bmatrix}
        F_1 \\
        F_2 \\
        F_3 \\
        F_4
    \end{bmatrix}
\end{equation}

Assuming forces $F_i$ in each $i$ wheel as a combination of two forces that maintain the robot's stability during its movement: $F_{wi}$ is the reaction between each wheel and the ground, and $f_{wi}$ is the friction between the small rollers and the ground \cite{Li:2014}. The first force is related to the wheel speed, the normal force in the wheel, and the robot's movement in the $x$ axis, while the second force is related to the friction between the small rollers and the ground and the robot's movement in the $y$ axis.

The robot dynamics model helps to prevent wheel slippage during the acceleration by calculating the maximum acceleration in each direction. The robot's maximum speeds and other dynamic parameters are in table \ref{table:kin1}. Additional parameters were found with the method described in \cite{Conceicao:2009}.

Solving equation (\ref{eq:dyn1}) for the maximum speeds and considering the robot's center of mass is with a $\Delta x$ displacement from the geometric robot's center in the $x$ axis. The maximum acceleration in each direction are given by equation (\ref{eq:dyn2}):

\begin{equation}\label{eq:dyn2}
    \begin{matrix}
        \Ddot{x}_{max} = 5.13\;m/s^2\\
        \Ddot{y}_{max} = 4.55\;m/s^2\\
        \Ddot{\theta}_{max} = 26.91\;rad/s^2
    \end{matrix}
\end{equation}

Thus, there is a research gap concerning the development of strategies for fast design and tuning of an OMR controller considering a multi-robot dynamic environment and size restrictions.

 M1 Status: Estimated using TFEST                                 
Fit to estimation data: 65.76%, FPE: 23.5694  
 
M2 Status: Estimated using TFEST Fit to estimation data: 65.44%, FPE: 24.4209

M3 Status: Estimated using TFEST Fit to estimation data: 64.9%, FPE: 26.8247

M4 : Estimated using TFEST Fit to estimation data: 65.54%, FPE: 25.6002

\begin{figure}%
\centering
\includegraphics[width=0.5\textwidth]{imgs/9_mprs1.png}
\caption{Motor response to an MPRS input signal.}
\label{fig:mprs1}
\end{figure}


M1 Status: Estimated using TFEST Fit to estimation data: 91.09%, FPE: 47.3873

M2 Status: Estimated using TFEST Fit to estimation data: 91.22%, FPE: 47.380

M3 Status: Estimated using TFEST Fit to estimation data: 91.38%, FPE: 42.6482

M4 Status: Estimated using TFEST Fit to estimation data: 91.08%, FPE: 47.4194

\begin{table}
\centering
\caption{Identified transfer function with MPRS signal input.}\label{tab:model1}
\begin{tabular}{ccccc}
\hline
   & \multicolumn{2}{c}{\textbf{Discrete-time}} &  \multicolumn{2}{c}{\textbf{Continuous-time}} \\
\hline
 \textbf{Motor (\#)}   & \rule{0pt}{9pt} \textbf{Transfer Function}  &  \textbf{Fitting(\%)}&  \textbf{Transfer Function}  &  \textbf{Fitting(\%)}\\
\hline \hline 
    \rule{0pt}{9pt} $1$ & $\frac{21.64}{1 - 0.8482\cdot z^{-1}}$
      &  $80.97$ & $\frac{1.431e04}{s+102.4}$
      &  $81.85$\\\hline       
    \rule{0pt}{9pt} $2$ &  $\frac{26.83}{1 - 0.8266\cdot z^{-1}}$
      &  $83.69$ & $\frac{1.874e04}{s+123.4}$
      &  $85.28$\\\hline
    \rule{0pt}{9pt} $3$ &  $\frac{30.3}{1 - 0.8149\cdot z^{-1}}$
      &  $84.57$ & $\frac{2.183e04}{s+135.7}$
      &  $86.72$\\\hline
    \rule{0pt}{9pt} $4$ & $\frac{27.16}{1 - 0.8347\cdot z^{-1}}$
      &  $84.83$ & $\frac{1.852e04}{s+114.8}$
      &  $86.78$\\\hline        
      
\hline
\end{tabular}
\end{table}

and its control algorithm computes the values based on the desired response time, bandwidth, and transient response.

. It consists of three basic steps: data acquisition, model estimation, and model validation

Figure \ref{fig:robo1} shows the robot built under the SSL rules and used in this validation.

\begin{figure}[ht]
\centering
\includegraphics[width=.35\textwidth]{imgs/10_robo1.png}
\caption{Omnidirectional mobile robot used for validation.}
\label{fig:robo1}
\end{figure} 

The motor model estimation step is to obtain a discrete-time transfer function that best represents the motor's response over time. In this step we propose the use of a Multi-level Pseudo-Random Sequence (MPRS) signal within the motor operating range to identify its behavior instead of traditional Pseud-Random Binary Sequence (PRBS) to increase the model accuracy. We use the collected data in the real world to find the linearized motor model estimation following the methodology proposed by \cite{Hat:2015}. 

 while Figure \ref{fig:mprs1}b shows a fragment of the PRBS signal applied to the same motor with its respective response. 
 
 \multirow{3}{*}{PRBS}        & Number of Samples  &   4095 \\ 
         & Sampling Period  &   $0.05$ (sec)   \\ 
        & Binary Input  &   $[15;35]$   \\ \hline \
        
\begin{figure}[!ht]
\begin{center}
    \subfloat[]{\includegraphics[width=0.5\textwidth]{imgs/9_mprs_m1_zoom.png}}
    \subfloat[]{\includegraphics[width=0.5\textwidth]{imgs/12_prbs_m1_zoom.png}}
\end{center}
    \caption{Fragment with nine seconds of the motor response (in rad/s) to: (a) an MPRS input signal (in \% Duty Cycle); (b) a PRBS input signal (in \% Duty Cycle). }
    \label{fig:mprs1}
\end{figure}


\end{comment}
